Understanding Code Understandability Improvements in Code Reviews

Motivation: Code understandability is crucial in software development, as developers spend 58% to 70% of their time reading source code. Improving it can improve productivity and reduce maintenance costs. Problem: Experimental studies often identify factors influencing code understandability in controlled settings but overlook real-world influences like project culture, guidelines, and developers' backgrounds. Ignoring these factors may yield results with limited external validity. Objective: This study investigates how developers enhance code understandability through code review comments, assuming that code reviewers are specialists in code quality. Method and Results: We analyzed 2,401 code review comments from Java open-source projects on GitHub, finding that over 42% focus on improving code understandability. We further examined 385 comments specifically related to this aspect and identified eight categories of concerns, such as inadequate documentation and poor identifiers. Notably, 83.9% of suggestions for improvement were accepted and integrated, with fewer than 1% later reverted. We identified various types of patches that enhance understandability, from simple changes like removing unused code to context-dependent improvements such as optimizing method calls. Additionally, we evaluated four well-known linters for their ability to flag these issues, finding they cover less than 30%, although many could be easily added as new rules. Implications: Our findings encourage the development of tools to enhance code understandability, as accepted changes can serve as reliable training data for specialized machine-learning models. Our dataset supports this training and can inform the development of evidence-based code style guides. Data Availability: Our data is publicly available at https://codeupcrc.github.io.

==> unused-text.tex <==
However, many of these studies 
are inconclusive or controversial (e.g., ~\cite{Gopstein2017, Medeiros2019, Scanniello2013}) or have controversial results (e.g., ~\cite{Sharif2010,Binkley2013}).

Moreover, experimental results may not reflect what the developers believe to be the best coding alternatives. For example, previous works~\cite{Medeiros2019, Gopstein2017, langhout2021} found that visible block delimiters, placed in their own line, improve readability in C, C++, and Java programs~\cite{Oliveira2023}. However, style guides, which are written by developers for developers, do not comply with that. The Google Java Style Guide supports the finding by recommending the use of braces, even for empty or single statement blocks, but does not specify where to place them. However, the Linux Kernel Coding Style only agrees with this for functions and not for statements.
Furthermore, experimental results may not reflect what the developers care about and how developers actually improve their code for understandability purposes. Developers might even have different perceptions about what is the best code alternatives. For example, \autoref{fig:example_to_ternary} shows a code reviewer asking the developer to replace an \texttt{if} statement with a ternary operator to improve the understandability of the source code. In contrast, in the \autoref{fig:example_from_ternary}, the reviewer asks the developer to perform the inverse operation to improve understandability.



Considering only the code review comments about understandability improvements (Column: Yes), \numberToBeChecked{65.32\% ($663 \div 1,016$)} are about \textsc{Code}, \numberToBeChecked{15.47\%} about \textsc{JavaDoc}, \numberToBeChecked{8.47\%} about \textsc{Comments}, \numberToBeChecked{6.5\%} about \textsc{String literal}, and \numberToBeChecked{4.24\%} about \textsc{Others}.
The code review comments suggesting understandability improvements to \textsc{JavaDoc} and \textsc{Comment} comprise approximately 23.9\% of all analyzed understandability improvements. 
This is similar to the percentage of lines of code consisting of comments (JavaDoc or otherwise) in the reviewed versions of the \numberToBeChecked{2,401} source files associated to the analyzed code review comments, approximately 20\% of the lines of code of these files (excluding blank lines, as measured by CLOC\footnote{\url{https://github.com/AlDanial/cloc}}).   

